Adversarial Robustness as a Prior for Learned Representations

An important goal in deep learning is to learn versatile, high-level feature representations of input data. However, standard networks' representations seem to possess shortcomings that, as we illustrate, prevent them from fully realizing this goal. In this work, we show that robust optimization can be re-cast as a tool for enforcing priors on the features learned by deep neural networks. It turns out that representations learned by robust models address the aforementioned shortcomings and make significant progress towards learning a high-level encoding of inputs. In particular, these representations are approximately invertible, while allowing for direct visualization and manipulation of salient input features. More broadly, our results indicate adversarial robustness as a promising avenue for improving learned representations. Our code and models for reproducing these results is available at https://git.io/robust-reps .

==> benefits.tex <==
In the previous sections, we used $\ell_2$-robust training to achieve
representations that are composed of meaningful features, have a
human-aligned geometry, and admit model-faithful interaction methods.

Here, we demonstrate several additional benefits enabled by robust
embeddings and their increased human-alignment. We find that such embeddings provide us with natural methods for
input interpolations (Section~\ref{sec:interpolation}), feature
manipulation (Section~\ref{sec:exploration}), and sensitivity evaluation
(Section~\ref{sec:insights}).


==> insights.tex <==
The inner mechanisms of standard deep neural networks remain opaque to
human observers.  In response, significant work has been dedicated to
developing {\em interpretability techniques} that attempt to attribute
predictions of deep models to specific parts of the input in a
human-meaningful
manner~\cite{smilkov2017smoothgrad,sundararajan2017axiomatic,olah2017feature,olah2018building}.

\paragraph{The standard tradeoff between interpretability and model-faithfulness. }
The development of tools for interpreting (standard) deep learning models has
uncovered a fundamental tension between having explanations that are
faithful to the model and explanations that are meaningful to the humans
they are presented to. In particular, state-of-the-art methods for
interpretability must discard information that models are extremely
sensitive to---note, for example, that deep learning models are highly
sensitive to adversarial perturbations, but all successful interpretability
techniques suppress these perturbations from visualizations due to their
lack of human-meaningfulness. 

Obtaining human-meaningful interpretations is most often accomplished
by enforcing ``human priors'' {\em at explanation
time}~\citep{olah2018building}. These
human undoubtedly improve the readability of model explanations, but are
often crippled by a lack of faithfulness to the underlying model they are
meant to interpret. For
example, recent
work~\cite{nie2018theoretical,adebayo2018sanity} shows that many
interpretation-time priors result in model interpretations that are
model- or data-\textit{indepdendent}, and hence inherently
unable to explain the predictions of the model.

\paragraph{Interpretation via robust representations.} We show that robust
representations enable a simple, regularization-free method getting
insights into the decisions of robust models. For any input image $x$, we
find the top $m$ (here we use $m=2$) components of the representation layer
that are most
activated by $x$ (appropriately weighted and scaled; c.f. Appendix~\ref{}
for details). We then magnify these coordinates in the input by performing the
feature addition objective described in Section~\ref{sec:exploration}.  
The resulting images are similar to the originals, but with the
highest-weight features accentuated. In addition to providing insight
about correct classifications (Figure~\ref{fig:closest_mis} right), these
images can also suggest {\em why} certain images are misclassified
(Figure~\ref{fig:closest_mis} left).
Again, performing a similar analysis for standard model requires
incorporating non-trivial human priors in order to make the result
human-meaningful (and hence sacrificing faithfulness to the underlying
model)~\cite{simonyan2013deep,yosinski2015understanding,olah2017feature,olah2018building}.

for {\em interpretation via perturbation}~\citep{fong2017interpretable}. Interpretation via
perturbation refers to a model explanation method wherein for an image $x$,
the model explanation consists of a similar image $x'$ (or several such
images) along with its (or their) classification(s)---by looking at the
qualitative differences between $x$ and $x'$ one can try to discern what
features the classifier was using to make its decision\footnote{This type of
interpretation can be seen as somewhat analogous to interpretation via
counterfactual generation in the context of causal inference.}. Existing
techniques for perturbation-based interpretation suffer from the
aforementioned tradeoff and must apply human priors at interpretation time
(e.g. using a pretrained generative model, regularization/post-processing,
etc.), or else end up with unintelligible model
explanations~\citep{fong2017interpretable,chang2018explaining,dabkowski2017real}. 

It turns out, however, that we can exploit robust representations to
generating perturbation-based explanations for robust models without
enforcing any priors at interpretation time. 


In Figure~\ref{fig:closest_mis}, accentuating the
highest-weight features reveals a natural transformation from the ear of a
monkey to the eye of a dog (top), from negative space to the face of a dog
(middle), and from the heads of two different fish to the two eyes of a single
frog, with a reed transforming into a mouth (bottom). These transformations
hint at the most sensitive directions of robust models on
misclassified inputs, thus providing insight into model decisions.

\begin{figure}[h!]
	\centering
	\includegraphics[width=1\textwidth]{./Figures/classification_features_IN.pdf}
	\caption{Accentuating the highest-weight features for correctly
	classified (right) and incorrectly (left) classified images. The
	highest-weight features are determined based
	on~\eqref{eq:interpretability_max}, and accentuated via the ``feature
    addition'' mechanism described in Section~\ref{sec:exploration}
    (Equation~\eqref{eq:clipped}). The resulting images appear to show
    plausible ways in which the images could have been
    classified/misclassified.}
    \label{fig:closest_mis}
\end{figure}


==> inversion_requires.tex <==
\begin{equation}
    \label{eq:recovery}
    x_1' = \min_{\|\delta\|_2 \leq \varepsilon} \|R(x_1 + \delta) - R(x_{2})\|,
\end{equation}
for a target image $x_2$ and a starting image $x_1$. This objective is
similar to the inversion objective~\eqref{eq:motivation_objective}, with the
added restriction that $\delta$ have small norm, meaning that the resulting
image $x_1'$ must look similar to $x_1$ (and thus different from $x_2$, which
was sampled independently. 

To accomplish this, given any input image, we start by
computing the largest-magnitude coordinates of the corresponding
representation, weighted by the linear classifier in the last layer (mapping from representations to logits). More
precisely, for an input $x$ with predicted class $c \in \{1\ldots C\}$ we
find:
\begin{equation}
    \label{eq:interpretability_max}
    \text{top-k}\left\{ R(x)_i \cdot W_{ic}\quad \forall\quad i \right\},
\end{equation}
where $W$ is the linear layer mapping from representations to logits.


==> old_benefits.tex <==
The promise of deep networks is that they learn meaningful representations of
the input.
In particular, they map inputs from the ambient space to a latent space where
$\ell_2$ distance is a meaningful metric of similarity and different classes are
linearly separable~\cite{xx}.
Moreover, these representations are particularly useful as they transfer
across tasks.
Learned representations for one task can be used for a different task, e.g. by
training a linear classifier on that representation (known as transfer
learning~\cite{xx}).

At the same time, learned representation are often of limited utility for the
task itself.
In particular, they suffer from two crucial shortcomings:
a) they are not directly related to human-visible concepts,
b) information about the geometry of the representation space cannot be
translated to information about the input space.
At the heart of both issues is the fact that deep learned representations are
extremely {\em brittle}.
That is, imperceptible changes in the input of a deep network cause large
changes in the representation of the inputs.
These changes are sufficient to cause misclassification, a phenomenon known as
adversarial examples~\cite{xx, xx}.
Conceptually, the brittleness of learned representations represents a complete
disconnect between input and representation space from a human perspective.
While inputs are mapped to representations that allow for correct
classification, these representations do not correspond necessarily to
semantically correct inputs.

We will bridge this gap by utilizing {\em adversarially \syss}.
The goal is to obtain representations that are robust to small changes of the
input space.
As a result, these representations are relevant in a neighborhood around the
input.
While such perturbations have been mostly considered in the context of ML
security~\cite{xx}, we will show how they are a fundamental property of a model
that is desired in any context.

We will show how \syss can be directly leveraged to obtain a range of desirable
properties.
In particular, studying the sensitivity of class scores and individual
representation components provides us with insights about how the model makes
its predictions.
Moreover, \syss allow us to perform semantically meaningful input manipulation
by utilizing the latent space structure.

